Bayesian ECG reconstruction using denoising diffusion generative models

In this work, we propose a denoising diffusion generative model (DDGM) trained with healthy electrocardiogram (ECG) data that focuses on ECG morphology and inter-lead dependence. Our results show that this innovative generative model can successfully generate realistic ECG signals. Furthermore, we explore the application of recent breakthroughs in solving linear inverse Bayesian problems using DDGM. This approach enables the development of several important clinical tools. These include the calculation of corrected QT intervals (QTc), effective noise suppression of ECG signals, recovery of missing ECG leads, and identification of anomalous readings, enabling significant advances in cardiac health monitoring and diagnosis.

==> def.tex <==
\def\rmd{\mathrm{d}}
\def\pP{\mathbb{P}}
\def\noise{\varepsilon}
\def\pE{\mathbb{E}}
\def\pV{\mathbb{V}}
\def\ltrstate{\mathbf{x}}
\def\eqdef{:=}
\def\baseset{\Omega}
\def\basesigma{\mathcal{F}}
\def\baseprob{\mathbb{P}}
\def\eqsp{\,}
\def\1{\mathbbm{1}}
\def\dimx{{\mathsf{d}_x}}
\def\dimz{d_z}
\def\dimy{{\smash{\overline{d}}}}
% \def\dimtr{{\smash{\overline{d}}}}
\def\dimtr{{\mathsf{d}_{\ltrmeas}}}
\newcommand{\numsqrt}[1]{\smash{#1}^{1/2}}
\def\dimorig{\mathsf{d}_y}
% \def\dimb{\smash{\underline{d}}}
\def\dimb{\mathsf{b}}
\def\trmeas{\mathbf{Y}}
\def\ltrmeas{\mathbf{y}}
\def\ormeas{Y}
\def\lmeas{y}
\def\revmeas{\overleftarrow{Y}}
\def\state{X}
\def\diffltrmeas{\mathsf{\ltrmeas}}
\def\trstate{\mathbf{X}}
\def\rset{\mathbb{R}}
\def\nset{\mathbb{N}}
\def\nsetpos{\mathbb{N}_*}
\def\idm{\operatorname{I}}
\def\nlessc{\m{J}^0}
\newcommand{\topvec}[1]{\overline{#1}}
\newcommand{\botvec}[1]{\underline{#1}}
\def\nyc{\m{J}}
\def\inflationstd{\kappa}
\def\model{\ensuremath{\operatorname{ECGDiff}}}

\newcommand{\nofrac}[2]{#1/#2}
% \newcommand{\m}[1]{\operatorname{#1}}
\newcommand{\m}[1]{\mathrm{#1}}
\newcommand{\cat}[2]{{#1}^{\scriptscriptstyle\frown}#2}
% \newcommand{\cat}[2]{\big[#1:#2\big]}
\newcommand{\vect}[1]{\mathbf{#1}}
% \DeclareMathOperator*{\argmin}{argmin}
\def\gauss{\mathcal{N}}
\def\noise{\varepsilon}
\def\iid{\overset{\mathrm{i.i.d.}}{\sim}}
\def\R{\mathbb{R}}
\def\bV{\mathbf{V}}
\DeclareMathOperator*{\argmax}{argmax}
\def\bY{\mathbf{Y}}
\def\stateperp{\mathbf{x}^\perp}
\def\stateperp{\bm{\xi}^\perp}
\def\invX{\xi}
\def\perpstate{\bm{\xi}}
\def\parallelstate{\bm{\zeta}}
\def\datadistr{\fwmarg{\operatorname{data}}{}}
\def\refmeas{\lambda}
\def\param{\theta}
\def\cov{\mathrm{\mathbb{C}ov}}
\def\sigalgebra{\mathcal{B}}
\def\normpdf{\mathcal{N}}
\def\pdf{p.d.f.}
\def\normdist{\mathcal{N}}
\def\normconst{\mathcal{Z}}
\def\sumweights{\Omega}
\def\boundedfunc{\mathbb{F}_b}
\def\bigo{\mathcal{O}}
\def\eigSigmay{\sigma^y}
\def\eigA{\sigma^A}
\def\id{\mathbf{I}}
\def\categorical{\mathrm{Cat}}
\def\ouralgorithm{\algo}
\def\motif{\mathcal{M}}
\def\scaffold{\mathcal{S}}
\def\bridgemean{\boldsymbol{\mu}}
\def\bridgevar{\boldsymbol{v}^2}
\def\bwmean{\mathsf{m}}
\def\bwmeanV{\mathfrak{m}}
\def\tbwmean{\overline{\mathsf{m}}}
\def\bbwmean{\underline{\mathsf{m}}}
\def\IPstdnoise{\sigma_\ltrmeas}

\newcommand{\card}[1]{|#1|}
\newcommand{\eigsigy}[1]{\sigma_{y, #1}}
\newcommand{\twodvect}[2]{(#1, #2)}
\newcommand{\xblock}[2]{x^{B_{#2}} _{#1}}
\newcommand{\filtration}[1]{\mathcal{F}_{#1}}
\newcommand{\fwdker}[3]{\overrightarrow{\mathbf{B}}_{#1}(#2 #3)}
\newcommand{\uweight}[2]{\widetilde{\omega}^{#1} _{#2}}
\newcommand{\weight}[2]{\omega^{#1} _{#2}}
\newcommand{\wratio}[3]{\frac{\tilde{\omega}^{#1} _{#2}(#3)}{\Omega^N _{#2}}}
\newcommand{\kldivergence}[2]{\ifthenelse{\equal{#2}{}}{\mathsf{KL}}{\mathsf{KL}({#1} \parallel {#2})}}
\def\particle{\xi}
\def\tparticle{\smash{\overline{\particle}}}
\def\bparticle{\smash{\underline{\particle}}}
\newcommand{\iparticle}[2]{x^{#1} _{#2}}
\newcommand{\mset}[2]{\R^{#1 \times #2}}
\newcommand{\X}[1]{X_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{}}{\mathbf{x}}{\mathbf{x}_{#1}}}
\newcommand{\important}[1]{\textcolor{red}{#1}}
\newcommand{\statevar}[1]{\mathbf{x}_{#1}}
% \newcommand{\statevar}[1]{\ifthenelse{\equal{#1}{1}}{\mathbf{x}}{\mathbf{x}_{#1}}}
% \newcommand{\statevar}[1]{\mathbf{x}_{#1}}
\newcommand{\Y}[1]{Y_{#1}}
\newcommand{\revX}[1]{\overset{{}_{\leftarrow}}{X} _{#1}}
\newcommand{\revY}[1]{Y_{#1}}
\newcommand{\W}[1]{W_{#1}}
\newcommand{\condprob}[2]{\baseprob\left(#1|#2\right)}
\newcommand{\score}[3]{\mathbf{s}_{#1}(#2, #3)}
\newcommand{\zerom}[2]{\mathbf{0}_{#1, #2}}
\def\noisestd{\sigma}
\def\tbw{...}
\def\orthdatadistr{\tilde{\pi}_{*}}
\def\orthmarginal{\smash{\bwmarg{0}{}^{_{\m{V}}}}}
\newcommand{\alphacumprod}[2]{\ifthenelse{\equal{#2}{}}{\bar{\alpha}_{#1}}{\bar{\alpha}_{#1,#2}}}
\newcommand{\fwsigma}[2]{\sigma_{#1,#2}}
 \newcommand{\eric}[1]{\todo[color=blue!20]{{\bf E:} #1}}
 \newcommand{\erici}[1]{\todo[inline,color=blue!20]{{\bf E:} #1}}
\newcommand\gabriel[1]{\todo[color=green!20]{{\bf G:} #1}}
\newcommand\lisa[1]{\todo[color=red!20]{{\bf L:} #1}} 
\newcommand\syl[1]{\todo[color=red!60]{{\bf Syl:} #1}}
\newcommand\josselin[1]{\todo[color=yellow!20]{{\bf J:} #1}}
\newcommand\remi[1]{\todo[color=gray!20]{{\bf R:} #1}}
\newcommandx{\xpred}[2][2=]{\boldsymbol{\chi}^{#2} _{#1}}
\newcommandx{\bottomxpred}[2][2=]{\underline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommandx{\topxpred}[2][2=]{\overline{\boldsymbol{\chi}}^{#2} _{#1}}
\newcommand{\ndist}[2]{\mathcal{N}(#1, #2)}
\newcommand{\soset}[1]{\operatorname{SO}(#1)}
\newcommand{\tstatevar}[1]{\overline{\mathbf{x}} _{#1}}
\newcommand{\bstatevar}[1]{\underline{\mathbf{x}} _{#1}}
\newcommand{\tstate}[1]{\overline{\state} _{#1}}
\newcommand{\bstate}[1]{\underline{\state} _{#1}}
\newcommand{\tcr}[1]{\textcolor{red}{#1}}
\newcommand{\prior}[1]{p_{#1}}
% \newcommand{\proposal}[2]{p_{#1, #2}}
\newcommand{\predstartprop}[2]{f_{#2}(#1)}
\newcommand{\epsprop}[2]{\ifthenelse{\equal{#1}{}}{\mathbf{e}^{#2}}{\mathbf{e}^{#2} (#1)}}
\newcommand{\vecidx}[3]{#1 _{#2}[#3]}
\newcommand{\expec}[2]{\mathbb{E}_{ #1}\left[#2\right]}
\newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{q} _{#1}}{\mathsf{q} _{#1}(#3|#2)}}
\newcommand{\revbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\infprocparam} _{#1}}{\smash{{q}}^{\infprocparam} _{#1}(#3|#2)}}
\newcommand{\idxrevbridge}[4]{\ifthenelse{\equal{#2}{}}{\smash{{q}}^{\sigma, #4} _{#1}}{\smash{{q}}^{\sigma, #4} _{#1}(#3|#2)}}
\newcommand{\trevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overline{q}}^{\sigma} _{#1}}{\smash{\overline{q}}^{\sigma} _{#1}(#3|#2)}}
\newcommand{\brevbridge}[3]{\ifthenelse{\isempty{#2}}{\underline{q}^{\sigma} _{#1}}{\underline{q}^{\sigma} _{#1}(#3|#2)}}
% \newcommand{\realrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\smash{\overset{{}_{\leftarrow}}{q}^{\sigma_*}} _{#1}}{\smash{\overset{{}_{\leftarrow}}{q}}^{\sigma_*} _{#1}(#3|#2)}}
\newcommand{\trealrevbridge}[3]{\ifthenelse{\equal{#2}{}}{\overline{\mathsf{q}}_{#1}}{\overline{\mathsf{q}} _{#1}(#3|#2)}}
\newcommand{\bbridgeker}[3]{\mathsf{Q}_{#1}(#3|#2)}
\newcommand{\sumweight}[1]{\Omega^N _{#1}}
\newcommand{\proposal}[2]{\overleftarrow{q}_{#1,#2}}
\newcommand{\bwproposal}[1]{\overleftarrow{Q}^{#1}}
\newcommand{\ouproposal}[1]{\overrightarrow{P}^{#1}}
\newcommand{\bridge}[4]{{\ifthenelse{\equal{#3}{}}{p^{#2} _{#1}}{p^{#2} _{#1}(#3, #4)}}}
\newcommand{\outrans}[3]{\ifthenelse{\equal{#2}{}}{\overrightarrow{m}_{#1}}{\overrightarrow{m}_{#1}(#2, #3)}}
% \newcommand{\bwtrans}[4]{\ifthenelse{\equal{#3}{}}{\smash{\overset{{}_{\leftarrow}}{m}^{#1}} _{#2}}{\smash{\overset{{}_{\leftarrow}}{m}}^{#1} _{#2}(#4|#3)}}
\newcommand{\bwtrans}[4]{\ifthenelse{\equal{#3}{}}{p^{#1} _{#2}}{p^{#1} _{#2}(#4|#3)}}
\newcommand{\bwtransV}[4]{\ifthenelse{\equal{#3}{}}{\lambda^{#1} _{#2}}{\lambda^{#1} _{#2}(#4|#3)}}
\newcommand{\bbwtransV}[4]{\ifthenelse{\equal{#3}{}}{\underline{\lambda}^{#1} _{#2}}{\underline{\lambda}^{#1} _{#2}(#4|#3)}}
\newcommand{\bbwtrans}[4]{\ifthenelse{\equal{#3}{}}{\underline{p}^{#1} _{#2}}{\underline{p}^{#1} _{#2}(#4|#3)}}
\newcommand{\tbwtrans}[4]{\ifthenelse{\equal{#3}{}}{\overline{p}^{#1} _{#2}}{\overline{p}^{#1} _{#2}(#4|#3)}}
\newcommand{\bwmargparam}[3]{\ifthenelse{\equal{#2}{}}{{{\mathfrak{p}}}_{#1}^{#3}}{{{\mathfrak{p}}}^{#3} _{#1}(#2)}}
\newcommand{\oldbwmargparam}[3]{\ifthenelse{\equal{#2}{}}{{{\mathsf{p}}}_{#1}^{#3}}{{{\mathsf{p}}}^{#3} _{#1}(#2)}}
\newcommand{\fwtrans}[3]{\ifthenelse{\equal{#2}{}}{q _{#1}}{q _{#1}(#3|#2)}}
\newcommand{\idxfwtrans}[4]{\ifthenelse{\equal{#2}{}}{q^{#4} _{#1}}{q^{#4} _{#1}(#3|#2)}}
\newcommand{\idxfwmarg}[4]{\ifthenelse{\equal{#2}{}}{{{\mathsf{q}}}^{#4} _{#1}}{{{\mathsf{q}}}^{#4} _{#1}(#3|#2)}}
\newcommand{\bfwtrans}[3]{\ifthenelse{\isempty{#2}}{\underline{q}_{#1}}{\underline{q}_{#1}(#3|#2)}}
\newcommand{\tfwtrans}[3]{\ifthenelse{\equal{#2}{}}{\overline{q} _{#1}}{\overline{q} _{#1}(#3|#2)}}
\newcommand{\idxtfwtrans}[4]{\ifthenelse{\equal{#2}{}}{\smash{\overline{q}}^{\sigma_\delta, #4} _{#1}}{\smash{\overline{q}}^{\sigma_\delta, #4} _{#1}(#3|#2)}}
\newcommand{\idxbwtrans}[4]{\ifthenelse{\equal{#2}{}}{p^{#4} _{#1}}{p^{#4} _{#1}(#3|#2)}}
\newcommand{\idxtbwtrans}[4]{\ifthenelse{\equal{#2}{}}{\smash{\overline{p}}^{#4} _{#1}}{\smash{\overline{p}}^{#4} _{#1}(#3|#2)}}
\newcommand{\bwmarg}[2]{\ifthenelse{\equal{#2}{}}{{{\mathsf{p}}}_{#1}}{{{\mathsf{p}}}_{#1}(#2)}}
\newcommand{\bwmargV}[2]{\ifthenelse{\equal{#2}{}}{{{\mathfrak{p}}}_{#1}}{{{\mathfrak{p}}}_{#1}(#2)}}
\newcommand{\bwoptmarg}[3]{\ifthenelse{\equal{#3}{}}{{{\mathsf{p}}}^{#2} _{#1}}{{{\mathsf{p}}}^{#2} _{#1}(#3)}}
\newcommand{\fwmarg}[2]{\ifthenelse{\equal{#2}{}}{{{\mathsf{q}}}_{#1}}{{{\mathsf{q}}}_{#1}(#2)}}
\newcommand{\initdistr}[3]{\ifthenelse{\equal{#2}{}}{\chi_{#1}}{\chi_{#1}(#2, #3)}}
% \newcommand{\bwopt}[4]{{\ifthenelse{\equal{#3}{}}{\overleftarrow{m}^{#2} _{#1}}{\overleftarrow{m}^{#2} _{#1}(#3 #4)}}}
\newcommand{\bwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{p^{#2} _{#1}(#4|#3)}}
\newcommand{\bbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\underline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\tbwopt}[4]{\ifthenelse{\equal{#3}{}}{p ^{#2} _{#1}}{\overline{p}^{#2} _{#1}(#4|#3)}}
\newcommand{\fwopt}[4]{\ifthenelse{\equal{#3}{}}{\overset{{}_{\rightarrow}}{m} ^{#2} _{#1}}{\smash{\overset{{}_{\rightarrow}}{m}}^{#2} _{#1}(#4|#3)}}
\newcommand{\ufilter}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\filter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\fwdfilter}[3]{{\ifthenelse{\equal{#3}{}}{\rho^{#2} _{#1}}{\rho^{#2} _{#1}(#3)}}}
\newcommand{\noisyfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi^{#2} _{#1}(#3)}}}
\newcommand{\noiselessfilter}[3]{{\ifthenelse{\equal{#3}{}}{\phi^{#2} _{#1}}{\phi _{#1}(#3 | #2)}}}
\newcommand{\pred}[3]{{\ifthenelse{\equal{#3}{}}{\eta^{#2} _{#1}}{\eta^{#2} _{#1}(#3)}}}
\newcommand{\bfilter}[3]{{\ifthenelse{\equal{#3}{}}{\Phi^{#2} _{#1}}{\Phi^{#2} _{#1}(#3)}}}
\newcommand{\normconstest}[1]{\gamma^N _{#1}}
\newcommand{\Qker}[2]{Q_{#1} ^{#2}}
\newcommand{\lawSMC}[1]{P^N _{#1}}
\newcommand{\lawcSMC}[1]{\mathbf{P}^N _{#1}}
\newcommand{\anc}[2]{\smash{I^{#1} _{#2}}}
\newcommand{\ianc}[2]{a^{#1} _{#2}}
\newcommand{\iancanc}[2]{b^{#1} _{#2}}
\newcommand{\pot}[3]{\ifthenelse{\equal{#3}{}}{\smash{g^{#2} _{#1}}}{\smash{g^{#2} _{#1}}(#3)}}
\newcommand{\dubpot}[3]{\ifthenelse{\equal{#3}{}}{G^{#2} _{#1}}{G^{#2} _{#1}(#3)}}
\newcommand{\fwfilter}[1]{\rho^{\ltrmeas} _{#1}}
% \newcommand{\dforward}[1]{\overrightarrow{m}_{#1}}
% \newcommand{\dbackward}[1]{\overleftarrow{m}_{#1}}
% \newcommand{\pot}[1]{g_{#1}}
% \newcommand{\optforward}[1]{\overrightarrow{p _{#1}}}
% \newcommand{\optbackward}[1]{\overleftarrow{p _{#1}}}
\newcommand{\couplepot}[1]{\mathrm{G}_{#1}}
\newcommand{\intvect}[2]{[#1:#2]}
\def\pathmforward{\overrightarrow{\lambda}}
\def\pathmbackward{\overleftarrow{\lambda}}
\newcommand{\assp}[1]{(\textbf{A}\textbf{#1})}
\newcommand{\clipleb}[3]{\nu^{#2} _{#1}(#3)}
\newcommand{\noisytrans}[3]{\ifthenelse{\equal{#2}{}}{\mathsf{P}_{#1}}{\mathsf{P}_{#1}(#3|#2)}}
\def\algo{\texttt{MCGdiff}}
\def\ddrm{\texttt{DDRM}}
\def\dps{\texttt{DPS}}
\def\smcdiff{\texttt{SMCdiff}}
\def\ddim{\texttt{DDIM}}
\def\rnvp{\texttt{RNVP}}
\def\dimg{d}
%\newcommand{\chunk}[3]{{#1}_{#2}^{#3}}
\newcommand{\chunk}[3]{#1_{#2:#3}}
\newcommand{\pchunk}[3]{#1 ^{#2:#3}}
\newcommand{\philter}[2]{\phi_{#1} ^{#2}}
\def\Id{\mathrm{I}}
\def\lstate{x}
\def\ltopstate{\overline{x}}
\def\lbottomstate{\underline{x}}
\def\ltopstate{\overline{x}}
\def\lbottomstate{\underline{x}}
\def\topstate{\smash{\overline{X}}}
\def\bottomstate{\underline{X}}
\def\trtopstate{\smash{\overline{\mathbf{X}}}}
\def\trbottomstate{\underline{\mathbf{X}}}
\def\ltrtopstate{\smash{\overline{\mathbf{x}}}}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\def\ltrbottomstate{\underline{\mathbf{x}}}
\newcommandx\sequence[3][2=,3=]
{\ifthenelse{\equal{#3}{}}{\ensuremath{\{ #1_{#2}\}}}{\ensuremath{\{ #1_{#2} \}_{#2 \in #3}}}}
\newcommand\projidx[3]{\ifthenelse{\equal{#2}{}}{#1^{\setminus #3}}{#1^{\setminus #3}_{#2}}}
\newcommand\insertidx[3]{#1^{#2, #3}}
\newcommand{\nf}[1]{\mathsf{f}_{#1}}
\def\varexpltrans{\rho^2}
\newcommand{\vestdker}[1]{\rho_{#1}}
\def\varexpl{{\upsilon}^2}
\def\stdexpl{{\upsilon}}
\def\varbridge{\Tilde{\upsilon}^2}
\newcommandx{\denoiser}[2][2=]{\mathcal{D}^{#2} _{#1}}
\def\indset{J}
\def\freeset{J_c}
\def\argmin{\operatorname{argmin}}
%\def\argmax{\operatorname{argmax}}
\def\residual{r}
\def\npart{M}
\def\QT{\operatorname{QT}}
\def\RR{\operatorname{RR}}
\def\vefinalsigma{\upsilon_{\operatorname{max}}}
\newcommand\mhdist[2]{\ifthenelse{\equal{#2}{}}{d_{\operatorname{MH}}}{d_{\operatorname{MH}}(#1; #2)}}
\def\biggervarset{\mathcal{V}}
\def\enddiff{K}
\def\emnsteps{\operatorname{L}}
\def\dimyt{\operatorname{T}_{y}}
\def\dimys{\operatorname{S}_{y}}
\def\nmle{N_{\operatorname{MLE}}}
\def\lrmle{\gamma}
\def\infprocparam{\eta}
\def\indmapl{\iota_{\operatorname{l}}}
\def\indmapt{\iota_{\operatorname{t}}}
\newcommand{\fnet}[1]{\operatorname{F}_{#1}}
\def\stddata{\sigma_{\operatorname{data}}}
\def\cin{\operatorname{c}_{\operatorname{in}}}
\def\cout{\operatorname{c}_{\operatorname{out}}}
\def\cskip{\operatorname{c}_{\operatorname{skip}}}
\def\cnoise{\operatorname{c}_{\operatorname{noise}}}
\newcommand{\posenc}[1]{\operatorname{PosEnc}(#1)}
\def\paramem{\varphi}
\newcommand{\hlgabriel}[1]{
{%
    \sethlcolor{cyan}%
    \hl{#1}%
}
}
\newcommand{\exedout}{%
\begin{tikzpicture}
\path node (LL) {}
    ++ (0.25\textwidth, 0.25\textheight) node (UR) {}
    (LL -| UR) node (LR) {}
    (LL |- UR) node (UL) {};
\draw (LL) rectangle (UR) (LL) -- (UR) (UL) -- (LR);
\end{tikzpicture}%
}

\newcommand{\exedouttwo}{%
\begin{tikzpicture}
\path node (LL) {}
    ++ (0.25\textwidth, 0.25\textheight) node (UR) {}
    (LL -| UR) node (LR) {}
    (LL |- UR) node (UL) {};
\draw (LL) rectangle (UR) (LL) -- (UR) (UL) -- (LR);
\end{tikzpicture}%
}
\def\stdmeet{\tau}

==> header.tex <==
\usepackage{soul}
%\usepackage{generic}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}
\usepackage[pdftex]{graphicx}
\usepackage{textcomp}
\usepackage{url}
\usepackage{amsmath,amsfonts,bm}
\usepackage{algorithm}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{algpseudocode}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage[small,labelfont=bf,up,textfont=it,up,margin=0pt]{caption}
\usepackage{subcaption}
\usepackage{datatool}
\RequirePackage{times}
\usepackage[textwidth=4cm,textsize=footnotesize]{todonotes}
\usepackage{ifthen}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{array}
\usepackage{xargs}
\usepackage{xifthen}
\usepackage[linesnumberedhidden,ruled,vlined, algo2e]{algorithm2e}
\RequirePackage[colorlinks=true,linkcolor=blue,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage[nodisplayskipstretch]{setspace}
\usepackage{amssymb,amsmath,amscd,amsfonts,bbm,mathrsfs,yhmath}
\usepackage{mathtools}
\usepackage{comment}
% \usepackage[parfill]{parskip}
\usepackage{booktabs}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\usepackage{cleveref}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\input{def}
\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
 \usepackage[export]{adjustbox}

\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}
\usepackage{geometry}
\geometry{
  paper = letterpaper,
  margin = 1.15in,
  includehead,
  footskip = 1cm
}
\graphicspath{{images}}
\title{Bayesian ECG reconstruction using denoising diffusion generative models}
\author{Gabriel V. Cardoso, Lisa Bedin, Josselin Duchateau, Rémi Dubois, Eric Moulines.}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mcg_diff_ve.tex <==
\subsection{Proposal kernel and weights}
By using standard Gaussian conjugation formulas,  we obtain the following proposal kernel and weight functions introduced in~\cref{eq:smc_recursion}
    \begin{align*}
\bwopt{t}{\lmeas}{\lstate_{t+1}}{\lstate_t} &= 
\prod_{\ell \in \biggervarset_t}
\normpdf(\ltopstate_t;
\mathsf{k}_{t,l} \lmeas[l] + (1 - \mathsf{k}_{s,l}) \overline{\mu_{t+1}}[l], \varexpl_t \mathsf{k}_{t,l} )\\
&\times \bbwtrans{}{t}{\lstate_{t+1}}{\lbottomstate_t} \times
\prod_{\ell \notin \biggervarset_t}\tbwtrans{}{t}{\lstate_{t+1}}{\ltopstate_t[l]}\eqsp,\\
\uweight{}{0}(\ltopstate_1) &= \int \tbwtrans{}{t}{\lstate_{t+1}}{\ltopstate_{t}} \tfwtrans{t|0}{\lmeas}{\ltopstate_{t}} \rmd \lstate_{t} \big/ \tfwtrans{t+1|0}{\lmeas}{\ltopstate_{t+1}}  \\
 &=\frac{\prod_{\ell \in \biggervarset_t}\normpdf\left(\lmeas[l]; \overline{\mu_{t+1}}[l], \varbridge_{t+1} + \varexpl_t-\vecidx{\Sigma}{\lmeas}{\ell, \ell}\right)}{\normpdf\left(\lmeas; \ltopstate_{t+1}, \varexpl_{t+1} \right)} \eqsp,
\end{align*}
where 
\begin{align*}
    \mathsf{k}_{t,l}&=\frac{\varbridge_t-\vecidx{\Sigma}{\lmeas}{\ell, \ell}}{\varbridge_t+\varexpl_t}\eqsp,\\
\mu_{t+1}&=\boldsymbol{\mu}_{t+1}(\lstate_{t+1}, \denoiser{0|t+1}( \lstate_{t+1}))\eqsp.
\end{align*}


%For ease of notations, we refer to the estimated bridge mean as $\mu_t=\boldsymbol{\mu}_t(\lstate_t, \denoiser{0|t}( \lstate_t))$. 


\subsection{Oldies}

\begin{align*}
    \filter{t}{\lmeas}{\lstate} &\propto \pot{t}{\lmeas}{\ltopstate} \bwmarg{t}{\lstate}\eqsp, \quad 
    \pot{t}{\lmeas}{\ltopstate} \eqdef \prod_{\ell \in \biggervarset_t} \pot{t, \ell}{\vecidx{\lmeas}{}{\ell}}{\vecidx{\ltopstate}{}{\ell}}\eqsp, \\ \quad 
    &\pot{t, \ell}{\vecidx{\lmeas}{}{\ell}}{\vecidx{\ltopstate}{}{\ell}}=\gauss(\vecidx{\ltopstate}{}{\ell}; \vecidx{\lmeas}{}{\ell}, \varexpl_{t} - \vecidx{\Sigma}{\lmeas}{\ell, \ell})\eqsp, 
\end{align*}


We use \cref{eq:smc_recursion} to explain 
By replacing the distribbution $\phi$ by the empirical distribution we obtain the following relation

To sample 


\begin{itemize}
    \item Proposal Kernel:
    \begin{multline*}
\bwopt{s}{\lmeas}{\lstate_{s+1}}{\lstate_s} = \bbwtrans{}{s}{\lstate_{s+1}}{\lbottomstate_s} \normpdf(\ltopstate_s;
\mathsf{k}_s \lmeas + (1 - \mathsf{k}_s) \overline{\mu_{s+1}}, \varexpl_s \mathsf{k}_s )
\end{multline*}
where $\mathsf{k}_s=\frac{\varbridge_s}{\varbridge_s+\varexpl_s}$
and $\mu_{s+1}=\boldsymbol{\mu}_{s+1}(\lstate_{s+1}, \denoiser{0|s+1}( \lstate_{s+1}))$.
    \item The weight function $\uweight{}{s}$ is chosen as follows; 
$\uweight{}{0}(\ltopstate_1) = \tbwtrans{}{0}{\ltopstate_1}{\lmeas} \big/ \tfwtrans{1|0}{\lmeas}{\ltopstate_1}$, 
\begin{align*}
\label{eq:proposalkernel}
    \uweight{}{n-1}(\lstate_n) & = \int \bwtrans{}{n-1}{\lstate_{n}}{\lstate_{n-1}} \tfwtrans{n-1|0}{\lmeas}{\ltopstate_{n-1}} \rmd \lstate_{n-1} \\
    & = \normpdf\left(\lmeas; \boldsymbol{\mu}_{n}(\ltopstate_{n}, \overline{\denoiser{0|n}}( \lstate_{n})), \varbridge_{n} + \varexpl_s\right)
\end{align*} and for $s \in [1:n-2]$, 
\begin{equation}
\begin{aligned} 
    \label{eq:weightfunc}
    \uweight{}{s}(\lstate_{s+1}) =  \int \tbwtrans{}{s}{\lstate_{s+1}}{\ltopstate_{s}} \tfwtrans{s|0}{\lmeas}{\ltopstate_{s}} \rmd \lstate_{s} \big/ \tfwtrans{s+1|0}{\lmeas}{\ltopstate_{s+1}}  \\
    = \frac{\normpdf\left(\lmeas; \boldsymbol{\mu}_{s+1}(\ltopstate_{s+1},\overline{\denoiser{0|s+1}}( \lstate_{s+1})), \varbridge_{s+1} + \varexpl_s\right)}{\normpdf\left(\lmeas; \ltopstate_{s+1}, \varexpl_{s+1} \right)} \eqsp.
\end{aligned}
\end{equation}
\end{itemize}

The overall SMC algorithm targeting $\filter{0}{\ltrmeas}{}$ using the instrumental kernel \eqref{eq:proposalkernel} and weight function \eqref{eq:weightfunc} is summarized in \Cref{alg:algonoiseless}.



\subsection{Bayesian Inpainting and \algo\,}
In the Bayesian inpainting problem, we observe a part of state $\lmeas \in \rset^{\dimtr}$, which can be written as $\lmeas = (\vecidx{\lstate}{}{i})_{i \in \indset}$, where $\indset \subset \intvect{1}{\dimx}$ is a set of $\dimtr$ distinct observed state indexes and $\vecidx{\lstate}{}{i} \in \rset$ is the i-th coordinate of the vector $\lstate \in \rset^{\dimx}$. For $\lstate \in \rset^{\dimx}$ we denote by $\ltopstate \in \rset^{\dimtr}$ the coordinates in $\indset$ and we denote $\freeset$ the set of free (unobserved) indices and $\lbottomstate \in \rset^{\dimx - \dimtr}$ the vector of free coordinates. The posterior density defined only for the free coordinates $\lbottomstate$ is $\smash{\filter{0}{\lmeas}{\lbottomstate}} \propto \bwmarg{0}{\cat{\lmeas}{\lbottomstate}}$, where $\cat{}{}$ is the reconstruction operator based on the indices $\indset, \freeset$, i.e., for all $\lstate \in \rset^\dimx$, $\cat{\ltopstate}{\lbottomstate} = \lstate$.
To obtain approximate samples from $\smash{\filter{0}{\lmeas}{\lbottomstate}}$, we use the \algo\ algorithm introduced in \cite{cardoso2023monte}. \algo\ is a Sequential Monte Carlo (SMC) sampler that targets the sequence of distributions $\sequence{\fwtrans{t}{\lmeas}{\ltopstate_t}\oldbwmargparam{t}{\lstate_t}{}}[][\intvect{1}{n}]$ with a finite set of $N$ particles. One of the main advantages of \algo\ is that it is consistent, meaning that the Kullback-Leibler distance between \algo\ samples and the target posterior goes to 0 with a ratio of $N^{-1}$. %\gabriel{Est-ce qu'on spécifie ici le proposal kernel et poids?}
% \paragraph{Proposal kernel:}
% \[ 
% \bwopt{s}{\ltrmeas}{\ltrstate_{s+1}}{\ltrstate_s} = \bbwtrans{}{s}{\ltrstate_{s+1}}{\lbottomstate_s} \normpdf\left(\ltopstate_s; \mathsf{k}_s \ltrmeas + (1 - \mathsf{k}_s) \boldsymbol{\mu}_{s+1}(\ltopstate_{s+1}, \topdenoiser{0|s+1}(\m{V} \ltrstate_{s+1})), \varexpl_s \mathsf{k}_s \right) 
% \]
% where $\mathsf{k}_s=\frac{\sigma_s^2}{\sigma_s^2+\varexpl_s}$.

% \paragraph{Weight function:}
% The weight function $\uweight{}{s}$ is chosen as follows; 
% $\uweight{}{0}(\ltopstate_1) = \tbwtrans{}{0}{\ltopstate_1}{\ltrmeas} \big/ \tfwtrans{1|0}{\ltrmeas}{\ltopstate_1}$, 
% \begin{align*}
%     \uweight{}{n-1}(\ltrstate_n) & = \int \bwtrans{}{n-1}{\ltrstate_{n}}{\ltrstate_{n-1}} \tfwtrans{n-1|0}{\ltrmeas}{\ltopstate_{n-1}} \rmd \ltrstate_{n-1} \\
%     & = \normpdf\left(\ltrmeas; \boldsymbol{\mu}_{n}(\ltopstate_{n}, \topdenoiser{0|n}(\m{V} \ltrstate_{n})), \sigma_{n}^2 + \varexpl_s\right)
% \end{align*} and for $s \in [1:n-2]$, 
% \begin{equation}
% \begin{aligned} 
%     \label{eq:weightfunc}
%     \uweight{}{s}(\ltrstate_{s+1}) &=  \int \tbwtrans{}{s}{\ltrstate_{s+1}}{\ltopstate_{s}} \tfwtrans{s|0}{\ltrmeas}{\ltopstate_{s}} \rmd \ltrstate_{s} \big/ \tfwtrans{s+1|0}{\ltrmeas}{\ltopstate_{s+1}}  \\
%     & = \frac{\normpdf\left(\ltrmeas; \boldsymbol{\mu}_{s+1}(\ltopstate_{s+1}, \topdenoiser{0|s+1}(\m{V} \ltrstate_{s+1})), \sigma_{s+1}^2 + \varexpl_s\right)}{\normpdf\left(\ltrmeas; \ltopstate_{s+1}, \varexpl_{s+1} \right)} \eqsp,
% \end{aligned}
% \end{equation}

    
We introduce the following auxiliary kernel, that we explicit using usual Gaussian operations~\cite{}
\begin{equation}
\begin{aligned}
\label{eq:proposal_kernel}
&\bwopt{t}{\lmeas}{\lstate_{t+1}}{\lstate} = \frac{\pot{t}{\lmeas}{\ltopstate}\bwtrans{}{t|t+1}{\lstate_{t+1}}{\lstate}}{L(\lstate_{t+1}, y)}\\
& = \bbwtrans{}{t}{\lstate_{t+1}}{\lbottomstate} \normpdf(\ltopstate;
\mathsf{k}_t \lmeas + (1 - \mathsf{k}_t) \overline{\mu_{t+1}}, \varexpl_t \mathsf{k}_t )\eqsp,
\end{aligned}
\end{equation}
where $L(\lstate_{t+1}, y)$ is the normalization constant and $\mathsf{k}_t=\frac{\varbridge_t}{\varbridge_t+\varexpl_t}$
and $\mu_{t+1}=\boldsymbol{\mu}_{t+1}(\lstate_{t+1}, \denoiser{0|t+1}( \lstate_{t+1}))$.
We introduce the weight function
\begin{equation}
\begin{aligned} 
    \label{eq:weightfunc}
    \uweight{}{t}(\lstate_{t+1}) =  \frac{L(\lstate_{t+1},y)}{\pot{t+1}{\lmeas}{\ltopstate}}\eqsp.
\end{aligned}
\end{equation}



\begin{equation}
\begin{aligned} 
    \label{eq:weightfunc}
    \uweight{}{t}(\lstate_{t+1}) =  \int \tbwtrans{}{t}{\lstate_{t+1}}{\ltopstate_{s}} \tfwtrans{s|0}{\lmeas}{\ltopstate_{s}} \rmd \lstate_{s} \big/ \tfwtrans{s+1|0}{\lmeas}{\ltopstate_{s+1}}  \\
    = \frac{\normpdf\left(\lmeas; \boldsymbol{\mu}_{s+1}(\ltopstate_{s+1},\overline{\denoiser{0|s+1}}( \lstate_{s+1})), \varbridge_{s+1} + \varexpl_s\right)}{\normpdf\left(\lmeas; \ltopstate_{s+1}, \varexpl_{s+1} \right)} \eqsp.
\end{aligned}
\end{equation}
    \newpage

==> noiseless_example.tex <==
\subsection{Conditional generation details}
The overall SMC algorithm targeting $\filter{0}{\ltrmeas}{}$ using the instrumental kernel \eqref{eq:proposalkernel} and weight function \eqref{eq:weightfunc} is summarized in \Cref{alg:algonoiseless}.

\begin{algorithm2e}
    \caption{\algo\ ($\sigma = 0$)}
    \label{alg:algonoiseless}
    \SetKwInOut{KwInput}{input}\SetKwInOut{KwOutput}{output}
    \KwInput{Number of particles $N$}
    \KwOutput{$\pchunk{\particle _0}{1}{N}$}
    \tcp{\small{Operations involving index $i$ are repeated for each $i \in [1:N]$}}
    \BlankLine
    $\overline{z}^i _{n} \sim \normpdf(\mathbf{0}_{\dimtr}, \idm_{\dimtr}), \underline{z}^i _{n} \sim \normpdf(\mathbf{0}_{\dimb}, \idm_{\dimb})$;\\
    $\bparticle^i _n = \mathsf{k}_n \alpha_n ^{1/2} \ltrmeas + (1 - \alpha_n) \mathsf{k} _n \underline{z}^i _n$;\\
    Set $\particle^i _n = \cat{\overline{z}^i _n}{\bparticle^i _n}$;\\
    \For{$s \gets n-1:0$}{
        \If{$s = n-1$}{
            $\uweight{}{n-1}(\particle^i _n) = \normpdf\big(\alpha_{n-1}^{1/2} \ltrmeas; \boldsymbol{\mu}_{n}(\tparticle^i _{n}, \topxpred{0|n}( \particle^i _{n})), \sigma_{n}^2 + 1 - \alpha_s\big)$;
        }
        \Else{
            $\uweight{}{s}(\particle^i _{s+1}) = \frac{\normpdf\left(\alpha_{s}^{1/2} \ltrmeas; \boldsymbol{\mu}_{s+1}(\tparticle^i _{s+1}, \topxpred{0|s+1}( \particle^i _{s+1})), \sigma_{s+1}^2 + 1 - \alpha_s\right)}{\normpdf\left(\alpha_{s+1}^{1/2}\ltrmeas; \tparticle^i _{s+1}, 1 - \alpha_{s+1} \right)}$;
        }
        $\anc{i}{s} \sim \categorical\big(\{ \uweight{}{s}(\particle^{j} _{s+1}) / \sum_{k = 1}^N \uweight{}{s}(\particle^{k} _{s+1})\} _{j = 1} ^N \big)$;\\
        $\overline{z}^i _{s} \sim \normpdf(\mathbf{0}_{\dimtr}, \idm_{\dimtr}), \underline{z}^i _{s} \sim \normpdf(\mathbf{0}_{\dimb}, \idm_{\dimb})$;\\
        $\tparticle^i _s = \mathsf{k}_s \alpha^{1/2} _s \ltrmeas + (1 - \mathsf{k}_s) \boldsymbol{\mu}_{s+1}(\tparticle^{\anc{i}{s}} _{s+1}, \topxpred{0|s+1}(
        \particle^{\anc{i}{s}} _{s+1})) + (1 - \alpha_s) \mathsf{k}_s \overline{z}^i _{s}$;\\
        $\bparticle^{i}_{s} = \boldsymbol{\mu}_{s+1}(\tparticle^{\anc{i}{s}} _{s+1}, \topxpred{0|s+1}( \particle^{\anc{i}{s}} _{s+1})) + \sigma _{s+1} \underline{z}^i _{s}$;\\
        Set $\particle^i _s = \cat{\tparticle^i _s}{\bparticle^i _s}$;
    }
    \end{algorithm2e}

